MC-Search: Evaluating and Enhancing Multimodal Agentic Search with Structured Long Reasoning Chains

With the increasing demand for step-wise, cross-modal, and knowledge-grounded reasoning, multimodal large language models (MLLMs) are evolving beyond the traditional fixed retrieve-then-generate paradigm toward more sophisticated agentic multimodal retrieval-augmented generation (MM-RAG). Existing benchmarks, however, mainly focus on simplified QA with short retrieval chains, leaving adaptive planning and multimodal reasoning underexplored. We present MC-Search, the first benchmark for agentic MM-RAG with long, step-wise annotated reasoning chains spanning five representative reasoning structures. Each example specifies sub-questions, retrieval modalities, supporting facts, and intermediate answers, with fidelity ensured by HAVE (Hop-wise Attribution and Verification of Evidence), resulting in 3,333 high-quality examples averaging 3.7 hops. Beyond answer accuracy, MC-Search introduces new process-level metrics for reasoning quality, stepwise retrieval and planning accuracy. By developing a unified agentic MM-RAG pipeline, we benchmark six leading MLLMs and reveal systematic issues such as over- and under-retrieval and modality-misaligned planning. Finally, we introduce Search-Align, a process-supervised fine-tuning framework leveraging verified reasoning chains, showing that our data not only enables faithful evaluation but also improves planning and retrieval fidelity in open-source MLLMs.

==> Tables/Fix_Step_RAG.tex <==
% \begin{table}[t!]
% \renewcommand{\arraystretch}{1.08} 
% \small
% \centering
% \caption{\small Evaluation on the \textbf{Search-MM} benchmark under traditional RAG. Complete results with all models are reported in the Appendix \xy{TODO}.}
% \label{tab:twohop-fixed-rag-main}
% \resizebox{0.85\linewidth}{!}{%
% \begin{tabular}{llccc ccc}
% \toprule
% \multirow{2}{*}{\textbf{Reason Graphs}} & \multirow{2}{*}{\textbf{Model}} &
% \multicolumn{3}{c}{\makecell{\textbf{Accuracy}}} &
% \multicolumn{2}{c}{\makecell{\textbf{Alignment}}} &
% \multirow{2}{*}{\textbf{Golden F1 ($\uparrow$)}} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-7}
% & & F1($\uparrow$) & $\Delta$F1($\uparrow$) & LLJ($\uparrow$) & HPS($\uparrow$) & RD($\downarrow$) & \\
% \midrule

% % ===================== Text-Only =====================
% \multirow{3}{*}{Text Only Chain} 
% & Gemini-2.5-Pro    & 11.11 & 11.10 & 0.70 & \multirow{3}{*}{19.22} & \multirow{3}{*}{3.00} & 62.42 \\
% & Claude-3.7-Sonnet & 22.71 & 22.09 & 1.69 &                        &                        & 66.38 \\
% & InternVL3.5-8B    & 30.98 & 24.00 & 1.47 &                        &                        & 65.72 \\
% \midrule

% % ===================== Image-Initiated =====================
% \multirow{3}{*}{Image Initiated Chain} 
% & Gemini-2.5-Pro    & 6.06  & 1.21  & 0.25 & \multirow{3}{*}{21.11} & \multirow{3}{*}{2.42} & 69.83 \\
% & Claude-3.7-Sonnet & 21.72 & 21.10 & 1.72 &                        &                        & 72.62 \\
% & InternVL3.5-8B    & 31.26 & 21.64 & 1.24 &                        &                        & 63.86 \\
% \midrule

% % ===================== Parallel Multi-Images =====================
% \multirow{3}{*}{Parallel Multi-Images} 
% & Gemini-2.5-Pro    & 11.03 & 7.24  & 0.57 & \multirow{3}{*}{19.35} & \multirow{3}{*}{2.76} & 61.29 \\
% & Claude-3.7-Sonnet & 19.96 & 15.25 & 1.67 &                        &                        & 62.41 \\
% & InternVL3.5-8B    & 34.55 & 22.45 & 1.58 &                        &                        & 57.65 \\
% \midrule

% % ===================== Parallel Visual-Textual =====================
% \multirow{3}{*}{Parallel Visual-Textual} 
% & Gemini-2.5-Pro    & 4.03  & 3.39  & 0.21 & \multirow{3}{*}{10.87} & \multirow{3}{*}{3.18} & 53.46 \\
% & Claude-3.7-Sonnet & 15.80 & 13.87 & 1.45 &                        &                        & 58.51 \\
% & InternVL3.5-8B    & 23.83 & 17.14 & 1.14 &                        &                        & 58.82 \\
% \midrule

% % ===================== Text-Initiated =====================
% \multirow{3}{*}{Text Initiated} 
% & Gemini-2.5-Pro    & 17.60 & 2.19  & 1.03 & \multirow{3}{*}{26.72} & \multirow{3}{*}{1.90} & 55.94 \\
% & Claude-3.7-Sonnet & 25.55 & 23.77 & 2.20 &                        &                        & 57.13 \\
% & InternVL3.5-8B    & 30.80 & 17.94 & 1.47 &                        &                        & 38.70 \\
% \bottomrule
% \end{tabular}}
% \end{table}


\begin{table}[t!]
\renewcommand{\arraystretch}{1.1} 
\small
\centering
\caption{\small Evaluation on the \textsc{\name} benchmark under traditional RAG. Complete results with all models are reported in the Appendix. \xy{TODO}}
\label{tab:final-middle-row-number}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{llccc ccc}
\toprule
\multirow{2}{*}{\textbf{Reason Graphs}} & \multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\makecell{\textbf{Accuracy}}} &
\multicolumn{2}{c}{\makecell{\textbf{Alignment}}} &
\multirow{2}{*}{\textbf{Golden F1 ($\uparrow$)}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
& & F1($\uparrow$) & $\Delta$F1($\uparrow$) & LLJ($\uparrow$) & HPS($\uparrow$) & RD($\downarrow$) & \\
\midrule
\addlinespace[-0.001ex]
% ===================== Image-Initiated (red!5) =====================
\multirow{3}{*}{Image Initiated Chain} 
& \cellcolor{red!5}Gemini-2.5-Pro    & \cellcolor{red!5}6.06  & \cellcolor{red!5}1.21  & \cellcolor{red!5}0.25 & \cellcolor{red!5}      & \cellcolor{red!5}      & \cellcolor{red!5}69.83 \\
& \cellcolor{red!5}Claude-3.7-Sonnet & \cellcolor{red!5}21.72 & \cellcolor{red!5}21.10 & \cellcolor{red!5}1.72 & \cellcolor{red!5}21.11 & \cellcolor{red!5}2.42 & \cellcolor{red!5}72.62 \\
& \cellcolor{red!5}InternVL3.5-8B    & \cellcolor{red!5}31.26 & \cellcolor{red!5}21.64 & \cellcolor{red!5}1.24 & \cellcolor{red!5}      & \cellcolor{red!5}      & \cellcolor{red!5}63.86 \\
\addlinespace[-0.001ex]\midrule
\addlinespace[-0.001ex]
% ===================== Parallel Multi-Images (orange!7) =====================
\multirow{3}{*}{Parallel Multi-Images} 
& \cellcolor{orange!7}Gemini-2.5-Pro    & \cellcolor{orange!7}11.03 & \cellcolor{orange!7}7.24  & \cellcolor{orange!7}0.57 & \cellcolor{orange!7}      & \cellcolor{orange!7}      & \cellcolor{orange!7}61.29 \\
& \cellcolor{orange!7}Claude-3.7-Sonnet & \cellcolor{orange!7}19.96 & \cellcolor{orange!7}15.25 & \cellcolor{orange!7}1.67 & \cellcolor{orange!7}19.35 & \cellcolor{orange!7}2.76 & \cellcolor{orange!7}62.41 \\
& \cellcolor{orange!7}InternVL3.5-8B    & \cellcolor{orange!7}34.55 & \cellcolor{orange!7}22.45 & \cellcolor{orange!7}1.58 & \cellcolor{orange!7}      & \cellcolor{orange!7}      & \cellcolor{orange!7}57.65 \\
\addlinespace[-0.001ex]\midrule
\addlinespace[-0.001ex]
% ===================== Text-Initiated (yellow!10) =====================
\multirow{3}{*}{Text Initiated Chain} 
& \cellcolor{yellow!10}Gemini-2.5-Pro    & \cellcolor{yellow!10}17.60 & \cellcolor{yellow!10}2.19  & \cellcolor{yellow!10}1.03 & \cellcolor{yellow!10}      & \cellcolor{yellow!10}      & \cellcolor{yellow!10}55.94 \\
& \cellcolor{yellow!10}Claude-3.7-Sonnet & \cellcolor{yellow!10}25.55 & \cellcolor{yellow!10}23.77 & \cellcolor{yellow!10}2.20 & \cellcolor{yellow!10}26.72 & \cellcolor{yellow!10}1.90 & \cellcolor{yellow!10}57.13 \\
& \cellcolor{yellow!10}InternVL3.5-8B    & \cellcolor{yellow!10}30.80 & \cellcolor{yellow!10}17.94 & \cellcolor{yellow!10}1.47 & \cellcolor{yellow!10}      & \cellcolor{yellow!10}      & \cellcolor{yellow!10}38.70 \\
\addlinespace[-0.001ex]
\midrule
\addlinespace[-0.001ex]
% ===================== Parallel Visual-Textual (LavenderLight!20) =====================
\multirow{3}{*}{Parallel Visual-Textual} 
& \cellcolor{LavenderLight!20}Gemini-2.5-Pro    & \cellcolor{LavenderLight!20}4.03  & \cellcolor{LavenderLight!20}3.39  & \cellcolor{LavenderLight!20}0.21 & \cellcolor{LavenderLight!20}       & \cellcolor{LavenderLight!20}       & \cellcolor{LavenderLight!20}53.46 \\
& \cellcolor{LavenderLight!20}Claude-3.7-Sonnet & \cellcolor{LavenderLight!20}15.80 & \cellcolor{LavenderLight!20}13.87 & \cellcolor{LavenderLight!20}1.45 & \cellcolor{LavenderLight!20}10.87 & \cellcolor{LavenderLight!20}3.18 & \cellcolor{LavenderLight!20}58.51 \\
& \cellcolor{LavenderLight!20}InternVL3.5-8B    & \cellcolor{LavenderLight!20}23.83 & \cellcolor{LavenderLight!20}17.14 & \cellcolor{LavenderLight!20}1.14 & \cellcolor{LavenderLight!20}       & \cellcolor{LavenderLight!20}       & \cellcolor{LavenderLight!20}58.82 \\
\addlinespace[-0.001ex]\midrule
\addlinespace[-0.001ex]
% ===================== Text-Only (green!5) =====================
\multirow{3}{*}{Text Only Chain} 
& \cellcolor{green!5}Gemini-2.5-Pro    & \cellcolor{green!5}11.11 & \cellcolor{green!5}11.10 & \cellcolor{green!5}0.70 & \cellcolor{green!5}      & \cellcolor{green!5}      & \cellcolor{green!5}62.42 \\
& \cellcolor{green!5}Claude-3.7-Sonnet & \cellcolor{green!5}22.71 & \cellcolor{green!5}22.09 & \cellcolor{green!5}1.69 & \cellcolor{green!5}19.22 & \cellcolor{green!5}3.00 & \cellcolor{green!5}66.38 \\
& \cellcolor{green!5}InternVL3.5-8B    & \cellcolor{green!5}30.98 & \cellcolor{green!5}24.00 & \cellcolor{green!5}1.47 & \cellcolor{green!5}      & \cellcolor{green!5}      & \cellcolor{green!5}65.72 \\
[-0.4ex]\bottomrule
\end{tabular}}
\end{table}





==> Tables/Full_Table.tex <==
\begin{table*}[t!]
\centering
\caption{\small Evaluation of various models on the \textbf{Search-MM} benchmark under both \textbf{one-step RAG} and \textbf{agentic MM-RAG}. We report results across five reasoning graph categories. Best results are in \textbf{bold}, second-best are \underline{underlined}.}
\label{tab:graph-model-main}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{\textbf{Reasoning Graph}} & \multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\textbf{Answer Accuracy}} &
\multicolumn{2}{c}{\textbf{Chain Alignment}} &
\multirow{2}{*}{\textbf{Golden F1 ($\uparrow$)}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
& & F1 ($\uparrow$) & $\Delta$F1 ($\uparrow$) & LJ ($\uparrow$) & HPS ($\uparrow$) & RD ($\downarrow$) & \\
\hline

% ===================== Text-Only Chain =====================
\multirow{12}{*}{Text-Only Chain} & \multicolumn{7}{c}{\emph{Single-Step RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 27.50 & 27.48 & 1.69 & 19.22   & 3.00  & 61.90 \\
& Gemini-2.5-Flash  & 10.88 & 10.81 & 0.75 & 19.22 & 3.00 & 67.72 \\
& Gemini-2.5-Pro    & 11.11 & 11.10 & 0.70 & 19.22 & 3.00 & 62.42  \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\emph{Multimodal Agentic RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 30.96 & 30.94 & \underline{2.58} & \textbf{21.94} & 1.13 & \underline{61.90} \\
& Gemini-2.5-Flash  & \underline{34.03} & \underline{33.96} & 2.49 & 20.59 & \textbf{1.04} & \textbf{67.72} \\
& Gemini-2.5-Pro    & \textbf{34.47} & \textbf{34.46} & \textbf{2.66} & \underline{21.59} & \underline{1.07} & 62.42 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\hline

% ===================== Image-Initiated Chain =====================
\multirow{12}{*}{Image-Initiated Chain} & \multicolumn{7}{c}{\emph{Single-Step RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 29.37 & 27.06 & 0.83  & 21.36 & 3.00 & 68.29 \\
& Gemini-2.5-Flash  & 3.63 & -3.09 & 0.22 & 21.52 & 3.00 & 72.39 \\
& Gemini-2.5-Pro    & 2.34 & -2.51 & 0.13 & 21.52 & 3.00 & 69.83 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\emph{Multimodal Agentic RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini    & 36.49 & 34.18 & 2.63 & \underline{27.51} & \underline{1.46} & 68.29 \\
& Gemini-2.5-Flash  & \underline{44.10} & \underline{37.38} & \underline{3.01} & \textbf{31.46} & 2.91 & \textbf{72.39} \\
& Gemini-2.5-Pro    & \textbf{47.61} & \textbf{42.76} & \textbf{3.18} & 25.90 & \textbf{1.05} & \underline{69.83} \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\hline

% ===================== Multi-Images Fork =====================
\multirow{12}{*}{Multi-Images Fork} & \multicolumn{7}{c}{\emph{Single-Step RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 25.53 & 20.69 & 1.27 & 15.46 & 3.00 & 59.46 \\
& Gemini-2.5-Flash  & 6.49 & 1.58 & 0.56 & 15.38 & 3.00 & 64.40 \\
& Gemini-2.5-Pro    & 7.26 & 3.47 & 0.51 & 15.38 & 3.00 & 61.29 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\emph{Multimodal Agentic RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 24.00 & 19.16 & 2.13 & \underline{16.04} & 1.94 & \underline{59.46} \\
& Gemini-2.5-Flash  & \underline{36.80} & \underline{31.89} & \underline{2.35} & 13.45 & \underline{1.66} & \textbf{64.40} \\
& Gemini-2.5-Pro    & \textbf{40.37} & \textbf{36.58} & \textbf{2.76} & \textbf{18.68} & \textbf{1.40} & 61.29 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\hline

% ===================== Parallel Visual-Textual Fork =====================
\multirow{12}{*}{Parallel Visual-Textual Fork} & \multicolumn{7}{c}{\emph{Single-Step RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 15.20 & 14.87 & 0.77 & 14.95 & 3.00 & 53.98 \\
& Gemini-2.5-Flash  & 4.09 & 2.11 & 0.30 & 15.06 & 3.00 & 57.99 \\
& Gemini-2.5-Pro    & 4.04 & 3.40 & 0.32 & 15.06 & 3.00 & 53.46 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\emph{Multimodal Agentic RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 21.98 & 21.65 & 2.20 & \underline{15.00} & \underline{1.71} & \underline{53.98} \\
& Gemini-2.5-Flash  & \underline{29.92} & \underline{27.94} & \underline{2.58} & 11.43 & 2.70 & \textbf{57.99} \\
& Gemini-2.5-Pro    & \textbf{34.83} & \textbf{34.19} & \textbf{2.99} & \textbf{16.74} & \textbf{1.29} & 53.46 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\hline

% ===================== Text-Initiated Chain =====================
\multirow{12}{*}{Text-Initiated Chain} & \multicolumn{7}{c}{\emph{Single-Step RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini  & 24.67 & 13.02 & 1.43 & 26.67 & 3.00 & 49.47 \\
& Gemini-2.5-Flash  & 16.78 & -0.43 & 1.30 & 26.86 & 3.00 & 66.27 \\
& Gemini-2.5-Pro    & 14.51 & -0.90 & 1.22 & 26.86 & 3.00 & 55.94 \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\emph{Multimodal Agentic RAG}} \\
\cmidrule(lr){2-8}
& GPT-4o-Mini       & 30.11 & 18.46 & 2.41 & \textbf{27.18} & 1.76 & 49.47 \\
& Gemini-2.5-Flash  & \underline{43.55} & 26.34 & \underline{3.30} & \underline{25.20} & \underline{1.20} & \textbf{66.27} \\
& Gemini-2.5-Pro    & \textbf{45.30} & \textbf{29.89} & \textbf{3.62} & 19.51 & \textbf{0.95} & \underline{55.94} \\
& Claude-3.7-Sonnet & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\

\bottomrule
\end{tabular}%
}
\vspace{-0.65cm}
\end{table*}

==> Tables/Main_Exp.tex <==
\begin{table*}[t!]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{\small Evaluation of various models on the \textbf{Search-MM} benchmark when performing \textbf{agentic MM-RAG}. We report results across five reasoning graph categories. Best results are in \textbf{bold}, second-best are \underline{underlined}. \xy{TODO: change bold and underline when results are ready}}
\label{tab:graph-model-main}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{\textbf{Reasoning Graph}} & \multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\textbf{Answer Accuracy}} &
\multicolumn{2}{c}{\textbf{Chain Alignment}} &
\multirow{2}{*}{\textbf{Golden F1 ($\uparrow$)}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
& & F1 ($\uparrow$) & $\Delta$F1 ($\uparrow$) & LJ ($\uparrow$) & HPS ($\uparrow$) & RD ($\downarrow$) & \\
\hline
\rowcolor{green!5}
  & GPT-4o-Mini  & 30.96 & 30.94 & \underline{2.58} & \textbf{21.94} & 1.13 & \underline{61.90} \\
\rowcolor{green!5}
Text-Only Chain  &  Gemini-2.5-Flash   & \underline{34.03} & \underline{33.96} & 2.49 & 20.59 & \textbf{1.04} & \textbf{67.72} \\
\rowcolor{green!5}
  & Gemini-2.5-Pro     & \textbf{34.47} & \textbf{34.46} & \textbf{2.66} & \underline{21.59} & \underline{1.07} & 62.42 \\
\rowcolor{green!5}
 & Claude-3.7-Sonnet & 27.37 & 26.75 & 2.08 & 29.64 & 3.14 & 66.38 \\
% \rowcolor{green!5}
& InternVL3.5-8B & 34.82 & 27.84 & 2.45 & 21.81 & 2.15 &  \multirow{2}{*}{65.72} \\
&\textbf{\ + \textsc{\method}} & 38.45 & 31.47 & 2.68 & 20.54 & 1.28  & \\
% \rowcolor{green!5}
& Qwen2.5-VL-7B & 23.54 & 14.89 & 1.36 & 13.35 & 4.63 & \multirow{2}{*}{61.57} \\
&\textbf{\ + \textsc{\method}} & 37.54 & 28.89 & 1.99 & 19.04 & 0.98 & \\

\hline
\rowcolor{red!5}
& GPT-4o-Mini        & 36.49 & 34.18 & 2.63 & \underline{27.51} & \underline{1.46} & 68.29 \\
\rowcolor{red!5}
Image-Initiated Chain
& Gemini-2.5-Flash   & \underline{44.10} & \underline{37.38} & \underline{3.01} & \textbf{31.46} & 2.91 & \textbf{72.39} \\
\rowcolor{red!5}
& Gemini-2.5-Pro     & \textbf{47.61} & \textbf{42.76} & \textbf{3.18} & 25.90 & \textbf{1.05} & \underline{69.83} \\
\rowcolor{red!5}
& Claude-3.7-Sonnet & 37.80 & 33.09 & 2.60 & 27.31 & 1.18 & 72.62 \\
% \rowcolor{red!5}
& InternVL3.5-8B & 39.11 & 29.49 & 2.27 & 22.59  & 1.58 & \multirow{2}{*}{63.86} \\
&\textbf{\ + \textsc{\method}} & 42.27 & 32.65 & 2.53 & 32.49 & 0.94 & \\
& Qwen2.5-VL-7B & 26.30 & 8.65 & 1.34 & 16.51 & 4.04 & \multirow{2}{*}{60.95} \\
&\textbf{\ + \textsc{\method}} & 45.70 & 28.05 & 2.23 & 33.59 & 0.70 & \\

\hline
\rowcolor{orange!7}
& GPT-4o-Mini        & 24.00 & 19.16 & 2.13 & \underline{16.04} & 1.94 & \underline{59.46} \\
\rowcolor{orange!7}
Multi-Images Fork
& Gemini-2.5-Flash   & \underline{36.80} & \underline{31.89} & \underline{2.35} & 13.45 & \underline{1.66} & \textbf{64.40} \\
\rowcolor{orange!7}
& Gemini-2.5-Pro     & \textbf{40.37} & \textbf{36.58} & \textbf{2.76} & \textbf{18.68} & \textbf{1.40} & 61.29 \\
\rowcolor{orange!7}
& Claude-3.7-Sonnet & 29.78 & 27.85 & 2.07 & 19.43 & 1.45 & 62.41 \\
% \rowcolor{orange!7}
& InternVL3.5-8B & 33.08 & 20.98 & 2.13 & 16.02 & 2.25 & \multirow{2}{*}{57.65} \\
&\textbf{\ + \textsc{\method}} & 36.53 & 24.43  & 2.49 & 39.33 & 1.67 & \\
& Qwen2.5-VL-7B & 26.13 & 7.53 & 1.41 & 12.58 & 3.80 & \multirow{2}{*}{57.04} \\
&\textbf{\ + \textsc{\method}} & 38.01 & 19.41 & 2.11 & 41.20 & 1.16 & \\

\hline
\rowcolor{LavenderLight!20}
& GPT-4o-Mini        & 21.98 & 21.65 & 2.20 & \underline{15.00} & \underline{1.71} & \underline{53.98} \\
\rowcolor{LavenderLight!20}
Parallel Visual-Textual
& Gemini-2.5-Flash   & \underline{29.92} & \underline{27.94} & \underline{2.58} & 11.43 & 2.70 & \textbf{57.99} \\
\rowcolor{LavenderLight!20}
& Gemini-2.5-Pro     & \textbf{34.83} & \textbf{34.19} & \textbf{2.99} & \textbf{16.74} & \textbf{1.29} & 53.46 \\
\rowcolor{LavenderLight!20}
& Claude-3.7-Sonnet & 26.43 & 24.65 & 1.95 & 14.32 & 1.37 & 58.51 \\
% \rowcolor{LavenderLight!20}
& InternVL3.5-8B & 29.74 & 23.05 & 2.13 & 14.22 & 1.75 & \multirow{2}{*}{58.82} \\
&\textbf{\ + \textsc{\method}} & 30.72 & 24.03 & 2.29 & 23.55 & 1.45 & \\
& Qwen2.5-VL-7B & 22.94 & 14.32 & 1.33 & 10.09 & 3.93 & \multirow{2}{*}{55.76} \\
&\textbf{\ + \textsc{\method}} & 32.73 & 24.11 & 1.78 & 25.07 & 1.05 &  \\

\hline
\rowcolor{yellow!10}
& GPT-4o-Mini        & 30.11 & 18.46 & 2.41 & \textbf{27.18} & 1.76 & 49.47 \\
\rowcolor{yellow!10}
Text-Initiated Chain & Gemini-2.5-Flash   & \underline{43.55} & 26.34 & \underline{3.30} & \underline{25.20} & \underline{1.20} & \textbf{66.27} \\
\rowcolor{yellow!10}
& Gemini-2.5-Pro     & \textbf{45.30} & \textbf{29.89} & \textbf{3.62} & 19.51 & \textbf{0.95} & \underline{55.94} \\
\rowcolor{yellow!10}
& Claude-3.7-Sonnet & 36.10 & 17.36 & 2.63 & 25.09 & 1.12 & 57.13 \\
% \rowcolor{yellow!10}
& InternVL3.5-8B & 38.34 & 25.48 & 2.60 & 19.06 & 1.97 & \multirow{2}{*}{38.70} \\
&\textbf{\ + \textsc{\method}} & 40.87 & 28.01 & 2.59 & 37.82 & 1.44 & \\
& Qwen2.5-VL-7B & 31.47 & 14.34 & 1.66 & 17.02 & 3.80 & \multirow{2}{*}{39.86} \\
&\textbf{\ + \textsc{\method}} & 45.07 & 27.94 & 2.42 & 33.59 & 0.87 & \\
[-0.4ex]\bottomrule
\end{tabular}%
}
\vspace{-0.65cm}
\end{table*}




